State Estimation for Legged Robots Using Contact-Centric Leg Odometry

Our goal is to send legged robots into challenging, unstructured terrains that wheeled systems cannot traverse. Moreover, precise estimation of the robot's position and orientation in rough terrain is especially difficult. To address this problem, we introduce a new state estimation algorithm which we term Contact-Centric Leg Odometry (COCLO). This new estimator uses a Square Root Unscented Kalman Filter (SR-UKF) to fuse multiple proprioceptive sensors available on a legged robot. In contrast to IMU-centric filtering approaches, COCLO formulates prediction and measurement models according to the contact status of legs. Additionally, COCLO has an indirect measurement model using joint velocities to estimate the robot body velocity. In rough terrain, when IMUs suffer from large amounts of noise, COCLO's contact-centric approach outperforms previous IMU-centric methods. To demonstrate improved state estimation accuracy, we compare COCLO with Visual Inertial Navigation System (VINS), a state-of-the-art visual inertial odometry, in three different environments: flat ground, ramps, and stairs. COCLO achieves better estimation precision than VINS in all three environments and is robust to unstable motion. Finally, we also show that COCLO and a modified VINS can work in tandem to improve each other's performance.

==> sections/sec_arch.tex <==
% The core component of our framework is a SR-UKF that fuses IMU, joint encoders, and joint torque sensors. The SR-UKF estimates the full state of the robot based on sensors measurements. Comparing to previous works \cite{bloesch2013state}\cite{wisth2019robust}, we do not design our filter IMU-centric \cite{hitz2016state}. In IMU-centric approach, the filter is designed to have the prediction model integrates high frequency gyroscope reading and the measurement model corrects state with low frequency accelerometer reading \cite{madgwick2010efficient}, which follows a common filter design methodology that using sensors with higher frequency to update state in the prediction model, and using sensors with lower frequency as measurement \cite{maybeck1982stochastic}. While in our case, we separate sensor readings into the prediction model and the measurement model based on the foot contact status of legs. Therefore we call our framework contact-centric.

% Our proposed state estimation framework fuses multiple data using VINS-Fusion(site). We use IMU data from Hebi Modules, joint state from the joint encoder and joint torque data from serial elastic structure from the actuator. The sensed robot states from the Hebi Modules are fed into UKF state estimator to get the robot local state. In order to obtain global information and eliminate drifting error, we capture image from Intel realsense dual camera, which provides the environment point cloud to localize the camera position. The data from UKF and camera are then combined to calculate an accurate full robot state through VINS-Fusion. In the following sections, we will elaborate the UKF, VINS-Fusion and discuss thoughts on the design of this framework.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/state_estimation_flow2.eps}\label{fig:arch}
\caption{Block architecture of proposed state estimation framework.}
\end{figure}


%The platform on which we design and implement our state estimation framework is the hexapod Daisy made by Hebi Robotics. Each leg of the robot has three joints actuated by three Hebi X Modules. Every Hebi X Module contains a built-in IMU, a joint encoder, a motor controller and a serial elastic component \cite{pratt1995series}. The serial elasticity gives the motor the ability to sense joint torque precisely. How to leverage the joint torque information is one of the motivations for our state estimation framework. Additional to actuators and computing device in the Daisy robot, we add an Intel realsense camera to obtain camera images. 

%On the central computer of the Daisy we organize software using ROS. Other than necessary drivers that process sensor data, the robot software three main ROS nodes: robot\_control,
%robot\_ukf and
%vins. robot\_control is a gait control node sends control command to all Hebi X Modules. robot\_ukf contains the UKF odometry. vins is a modified verison of opensource VIO VINS-Fusion. The relationship of these nodes are shown in Figure \ref{fig:arch}. In Section \ref{sec:filter} we explain the algorithm in robot\_ukf. Then Section \ref{sec:vins} discuss how the UKF information can be used to improve VINS-Fusion. Section \ref{sec:exp} not only present the experiments we designed to test the performance of our state estimation framework but also briefly describe the control strategy we use to control the robot. 





==> sections/sec_filter.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/state_estimation_flow2.eps}\label{fig:arch}
\caption{Block architecture of proposed state estimation framework.}
\end{figure}


The UKF odometry estimates full state of the robot based on IMU, joint encoders, velocity sensor, and joint torque sensors measurements. A common filter design methodology is to sensors with higher frequency to update state in the prediction model, and use sensors with lower frequency as measurement \cite{maybeck1982stochastic}. In our case, these sensors are at the same frequency, so we separate them into the prediction model and measurement model based on the foot contact status of legs. Throughout the paper we will adopt the notation in \cite{murray2017mathematical} to represent vectors and rotations. A rotation matrix $R_{wc}$ changes the representation of a vector $p_c$ in CoM frame of the robot (c) into the world frame (w), denoted as
\begin{align}
    p_w = R_{wc}p_c.
\end{align}
We also denote the translation between world frame and COM frame as $t_{wc}$. The quaternion corresponds to the rotation matrix$R_{wc}$ is $q_{wc} = \begin{bmatrix} q_1 \ q_2 \ q_3 \ q_4 \end{bmatrix}$. Given a quaternion $q_{wc}$ and angular velocity $\omega_c = \begin{bmatrix} \omega_1 \ \omega_2 \ \omega_3 \end{bmatrix}^T$ in center of mass (CoM) frame, the update equation of the quaternion is
\begin{align}\label{eqn:quaternion}
    \dot{q}_{wc} = \frac{1}{2}q_{wc} \otimes 
    \begin{bmatrix}
        \omega_1 \\ \omega_2 \\ \omega_3 \\ 0
    \end{bmatrix}
\end{align}
in which $q \otimes p$ is one way to define quaternion product
6

\begin{align}
    q \otimes p = 
    \begin{bmatrix}
    p_4 & p_3 & -p_2 & p_1 \\
    -p_3 & p_4 & p_1 & p_2 \\
    p_2 & -p_1 & p_4 & p_3 \\
    -p_1 & -p_2 & -p_3 & p_4 \\
    \end{bmatrix}
    \begin{bmatrix}
    q_1 \\ q_2 \\ q_3 \\q_4
    \end{bmatrix}
\end{align}
The discretized version of Equation \ref{eqn:quaternion} is 
\begin{align}
   q_{wc(t+\Delta t)} = q_{wc(t)} + \frac{1}{2} q_{wc(t)} \otimes 
    \begin{bmatrix}
    \omega_c\Delta t \\ 0
    \end{bmatrix} 
\end{align}
For each individual leg, we model it as a fix base manipulator and calculate the transformation matrix between the foot tip of the leg (f) and the CoM frame of the robot using manipulator kinematics \cite{murray2017mathematical}. Given joint angles $\alpha$, the transformation is given by
\begin{equation}\label{eqn:fk}
  (R_{cf}, t_{cf}) = FK(\alpha)  
\end{equation}
Then position of the foot tip represented in world frame is
\begin{equation}
p_w = R_{wc}t_{cf} + t_{wc}
\end{equation}
Further, if the joint velocity sensor gives joint angular velocities $\dot{\alpha}$, then foot tip velocity represents in world frame is 
\begin{equation}\label{eqn:vel}
    \dot{p}_w = R_{wc}R_{cf} Jb(\alpha) \dot{\alpha}
\end{equation}
where $Jb()$ is the body Jacobian function.


\subsubsection{Unscented Kalman Filter}
We briefly describe the UKF algorithm \cite{wan2000unscented} to introduce necessary notations to facilitate discussion. Given a state estimation result $\hat{x}_t$ and its covariance $\hat{\textbf{P}}_t$, a list of sigma points is generated follows
\begin{align}
    \textbf{X}_{t} = \Big[ \hat{x}_t \quad \hat{x}_t+\gamma\sqrt{\hat{\textbf{P}}_t} \quad \hat{x}_t-\gamma\sqrt{\hat{\textbf{P}}_t} \Big]
\end{align}
Then, we pass the generated sigma points into the prediction model $f$
\begin{align*}
    \textbf{X}^*_{t+1|t} = f(\textbf{X}_{t})
\end{align*}
and intermediate state and covariance after \textit{prediction update} can be reconstructed as
\begin{align*}
    & \hat{x}^-_{t+1} = \sum W_i X^*_{i,t+1|t} \\
    & \hat{\textbf{P}}^-_{t+1} = \sum W_i [X^*_{i,t+1|t} - \hat{x}^-_{t+1}][X^*_{i,t+1|t} - \hat{x}^-_{t+1}]^T + Q
\end{align*}
where $Q$ is the prediction noise covariance matrix. Then, new sigma points based on intermediate state and covariance are generated for \textit{measurement update}
\begin{align}
   \textbf{X}_{t+1|t} = \Big[ \hat{x}^-_{t+1} \quad \hat{x}^-_{t+1}+\gamma\sqrt{\hat{\textbf{P}}^-_{t+1}} \quad \hat{x}^-_{t+1}-\gamma\sqrt{\hat{\textbf{P}}^-_{t+1}} \Big] 
\end{align}
and pass through the measurement model $h$
\begin{align*}
    \textbf{Y}_{t+1|t} = h(\textbf{X}_{t+1|t}).
\end{align*}
Then, we reconstructed the predicted measurement and corresponding covariances 
\begin{align*}
& \hat{y}^-_{t+1} = \sum W_i Y^*_{i,t+1|t} \\
& \hat{\textbf{P}}_{y_t,y_t} = \sum W_i [Y^*_{i,t+1|t} - \hat{y}^-_{t+1}][Y^*_{i,t+1|t} - \hat{y}^-_{t+1}]^T + R \\
& \hat{\textbf{P}}_{x_t,y_t} = \sum W_i [X^*_{i,t+1|t} - \hat{x}^-_{t+1}][Y^*_{i,t+1|t} - \hat{y}^-_{t+1}]^T 
\end{align*}
where $R$ is the measurement noise covariance matrix. Finally, given observed measurement $y_{t+1}$, Kalman gain and measurement update step are calculated by
\begin{align*}
& K_{t+1} = \hat{\textbf{P}}_{x_t,y_t}\hat{\textbf{P}}^{-1}_{y_t,y_t} \\
& \hat{x}_{t+1} = \hat{x}^-_{t+1} + K_{t+1} (y_{t+1} - \hat{y}^-_{t+1}) \\
& \hat{\textbf{P}}_{t+1} = \hat{\textbf{P}}^-_{t+1} - K_{t+1}\hat{\textbf{P}}_{y_t,y_t}K^T_{t+1}
\end{align*}
Then the filter continues with $K_{t+1}$ and $\hat{\textbf{P}}_{t+1}$ in next step. 

\subsubsection{State Definition}
With above notations, the KF state vector is defined as:
\begin{align}
    x = [r_w \quad v_w \quad q_{wc} \quad b_g \quad b_a \quad p_{w1} \dots  p_{wN} \quad c_1  \dots c_N]^T
\end{align}
where $r, v$ are the CoM position and velocity of the robot, $q$ is the quaternion representing orientation, $b_g$ and $b_a$ are estimated IMU sensor biases for gyroscope and accelerometer, and $p_1 \dots p_N$ are each of the foot positions. $r$, $v$, $q$, $p$ are all with respect to the world frame. $c_1 \dots c_N$ are the foot contact status of legs. The value $c_i$ is between $[0,1]$, representing the probability of the corresponding foot has contact with ground. The contact state is critical for the performance of the UKF odometry. 

\subsubsection{Prediction Model}
The inputs to the prediction model are angular velocity $\omega_c$ provided by the gyroscope, acceleration reading $a_c$ from the accelerometer and foot tip velocities $\dot{p}_{wi}$ ($i = 1\dots N$) calculated from joint sensors given in Equation \ref{eqn:vel}. 

During a small time increment $\Delta t$, the prediction model updates the state as follows:

\begin{align}
r_{t+1} = & r_{t} + v_{t}\Delta t \\
v_{t+1} = & v_{t} + \textbf{isAllTouch}(c_1\dots c_N)\cdot (q_t (a_c - b_{a,t})+g)\Delta t\\
q_{t+1} = & q_{t} + \frac{1}{2} q_{t} \otimes 
    \begin{bmatrix}
    (\omega_c - b_{g,t})\Delta t \\ 0
    \end{bmatrix} \\
b_{g,t+1} = & b_{g,t} \\
b_{a,t+1} = & b_{a,t} \\
p_{wi,t+1} = & p_{wi,t} +  \textbf{isSwing}(c_i)\dot{p}_{wi}\Delta t \\
c_{i,t+1} = & c_{i,t}
\end{align}

The term $\textbf{isAllTouch()}$ is a boolean function determines whether all feet are in contact with ground. In other words, the function returns 1 if all $c_i > \theta_{contact}$ where $\theta_{contact}$ is a predetermined threshold. The reason for having this function is to make sure the filter only update velocity using accelerometer when the robot body is in a stable status. Similarly, $\textbf{isSwing}()$ returns 1 if $c_i$ is less than threshold $\theta_{swing}$. This function ensures a leg only update its foothold position when the foot has no contact with the ground, in other ways, the leg is in ``swing`` status.

It is also important to adjust prediction noise covariance matrix Q according to foot contact status. Before each prediction update, the function $\textbf{isAllTouch()}$ and $\textbf{isSwing}()$ will be calculated first, and the elements in Q corresponding to foot positions of legs that are not swinging get value reduced 100 times because we are certain that they are not likely to move when they are standing on the ground. Further, if $c_i = 1$, the variance reduce another 100 times for $c_i = 1$ means we are pretty certain about the status of the foot being on the ground without moving or slipping.  

\subsubsection{Measurement Model}
The output of the measurement model $h(x)$ can be split into different parts:
$$
h(x) = 
\begin{bmatrix}
q_{wc}^T g_w + b_a \\
q_{wc}^T( r_w - p_{wi}) ,i = 1\dots N \\
v \\
\hat{c}_i ,i = 1\dots N 
\end{bmatrix}
$$

The first term is the commonly used gravity direction measurement method in complimentary filter \cite{madgwick2010efficient}. Its corresponding $y_{t+1}$ term is just $a_c$. However, as IMU shock will make the gravity direction measurement wrong. We only use this measurement when robot has all legs in contact with ground. This can be achieved by changing terms in the measurement noise covariance matrix R to have very large value when $\textbf{isAllTouch()}$ is not returning 1. In this way the Kalman gain will give relevant terms in the innovation small weight so it would not affect the estimated state. 

The second part, $q_{wc}^T( r_w - p_{wi})$, uses the forward kinematics of each leg as measurement as given in Equation \ref{eqn:fk}.

The third term is the body velocity of the robot. Its measurement comes from the joint angle and joint velocity sensors. For a leg stands on the ground, its joint movement reflects the motion of the body. So the foot tip velocity $\dot{p}_w$ is the reverse of the body velocity. Since there could be multiple legs stand on the ground, we can take the average of them to reduce measurement noise. So we define function $\textbf{isTouch}$() to get feet on the ground, then the velocity measurement is
$$
v = - q_{wc}\frac{1}{N_t}\sum^N_{i = 0}  \textbf{isTouch}(c_i)R_{wc}R_{cf} Jb(\alpha_i) \dot{\alpha_i}
$$
in which $N_t$ is number of legs that has contact with ground.

The last part of the measurement model is the contact status of each legs. We determine the contact status using joint torque sensors. The torques experienced on all joints are vector $\tau$, the torques can be transformed to get foot tip force F in world frame as 
$$
F = R_{wc}R_{cf}Jb^{-1}(\alpha)\tau
$$
We then use an empirical model to covert the tip force F to contact status. During the movement of the robot, we record the largest magnitude tip force as $\|F_{max}\|$. Then we calculate $\frac{\|F\|}{0.5\|F_{max}\|}$ and limit it within $[0,1]$ as the measurement of contact status. 


